MuTable (Music Table): Turn any surface into musical instrument

With the rise in pervasive computing solutions, interactive surfaces have gained a large popularity across multi-application domains including smart boards for education, touch-enabled kiosks for smart retail and smart mirrors for smart homes. Despite the increased popularity of such interactive surfaces, existing platforms are mostly limited to custom built surfaces with attached sensors and hardware, that are expensive and require complicated design considerations. To address this, we design a low-cost, intuitive system called MuTable that repurposes any flat surface (such as table tops) into a live musical instrument. This provides a unique, close to real-time instrument playing experience to the user to play any type of musical instrument. This is achieved by projecting the instrument's shape on any tangible surface, sensor calibration, user taps detection, tap position identification, and associated sound generation. We demonstrate the performance of our working system by reporting an accuracy of 83% for detecting softer taps, 100% accuracy for detecting the regular taps, and a precision of 95.7% for estimating hand location.

==> 000-abstract.tex <==
\begin{abstract}

\end{abstract}

==> 003-motivation_problemStatement.tex <==
\section{Motivation and Problem Statement}
\label{sec:motivation_problem}

% hypothesis, trends and how our problem addresses it. 

% Motivation+Concrete Problem Statement (need not be formal, only concrete).
% talk about the motivation for this project and for the following problem statement
%\subsection{Motivation}

% talk bout the problem statement
%\subsection{Problem Statement}

==> 005-timeline.tex <==
\section{Timeline}
\label{sec:timeline}


\begin{figure}[!htb]
\centering
\includegraphics[width=\linewidth] {Setup.PNG}
\caption{End-to-end workflow
}
\label{fig:Workflow}
\end{figure}


% Timeline/Expected Milestones for achieving your goals.
Our timeline is roughly to finish the first scope of the project (including the implementation and evaluation) by the midterm report deadline and to finish the second scope of the project (including the implementation and evaluation) by the final report deadline.
